A Workbench for Autograding Retrieve/Generate Systems

This resource paper addresses the challenge of evaluating Information Retrieval (IR) systems in the era of autoregressive Large Language Models (LLMs). Traditional methods relying on passage-level judgments are no longer effective due to the diversity of responses generated by LLM-based systems. We provide a workbench to explore several alternative evaluation approaches to judge the relevance of a system's response that incorporate LLMs: 1. Asking an LLM whether the response is relevant; 2. Asking the LLM which set of nuggets (i.e., relevant key facts) is covered in the response; 3. Asking the LLM to answer a set of exam questions with the response. This workbench aims to facilitate the development of new, reusable test collections. Researchers can manually refine sets of nuggets and exam questions, observing their impact on system evaluation and leaderboard rankings. Resource available at https://github.com/TREMA-UNH/autograding-workbench

==> evaluation.tex <==
\section{Experimental Evaluation (of the Evaluation Metric)}
\label{sec:evaluation}

\input{experimental-setup.tex}

\input{experimental-results.tex}

==> experimental-results.tex <==
\subsection{Results on \car{} / \tqa{}}

We first reproduce the experimental setup of the original EXAM method, using the \car{} collection and exam question banks from the \tqa{} dataset. 

As part of the exam grading, the FLAN-T5-large LLM is prompted to answer each exam question with every passage from the system response, which is then verified against the gold standard answer. 

The \examcover{} leaderboard generated using the \tqa{}-based \examcover{} approach is very similar to the official CAR-Y3 leaderboard (Table \ref{tab:car_leaderboard}). With the exception of the \texttt{ECNU\_ReRank1} method, the top 10 of the leaderboard is in exactly the same order. The Spearman rank measure is 0.94, Kendall $\tau$ is 0.84. Our approach outperforms the original EXAM metric significantly, obtaining a correlation comparable to MAP vs NDCG (cf. Table 1 in \citep{sander2021exam}).
%
This is visually confirmed in Figure \ref{fig:car-y3-leaderboard}.
%
While several methods obtain similar EXAM scores, these are indeed very similar systems with exactly the same score on the official leaderboard.

Given the distinct nature of our evaluation paradigm, a high inter-annotator agreement on the passage-level is not anticipated. Indeed, as shown in Table \ref{tab:car-tqa-binary-cohen}, the per-passage inter-annotator agreement is very low ($\kappa \approx 0.08$). In contrast to the leaderboard correlation, this demonstrates that a high agreement is not necessary to evaluate system quality correctly.


\begin{table}[]
    \centering
    \caption{\car{} leaderboards, ordered by \examcover{} on TQA questions. In terms of both Spearman's and Kendall's $\tau$ rank correlation coefficients, all our EXAM approaches obtain a better correlation with the official leaderboard than the original EXAM implementation. Note that some submitted systems were not included on the official leaderboard as they had not been assessed.}
    \label{tab:car_leaderboard}
\input{results/car-y3-leaderboard-correlation}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{results/car-y3-leaderboard.pdf}
    \caption{Comparing \car{} leaderboards, our EXAM metrics show strong correlation  with the official TREC leaderboard.    
    Methods are ordered by their official leaderboard rank (filled circles). Methods without official ranks are placed according to their TQA \examcover{} scores. Standard error bars given. For context, Sander's EXAM leaderboard (depicted as crosses) does not show as strong a correlation.}
    \label{fig:car-y3-leaderboard}
\end{figure}

\input{results/correlation--car-tqa-cc-corrected}


\input{results/correlation-car-naghmeh-self-rating}

\subsection{Results on \car{} with \genQ{}}

When switching to generated question banks, which do not have a correct answer key, we obtain comparable (albeit slightly lower) results. 

The leaderboard correlation (Table \ref{tab:car_leaderboard}, columns marked with \genQ{}) still obtain a very good correlation of Spearman $\approx 0.86$. According to Table \ref{fig:car-y3-leaderboard} (green lines), both the \examcover{} and \examqrels{} methods follow the trend of the official leaderboard. Interestingly, the system ICT-DRMMTKS denotes a positive outlier under both exam question banks.



\subsection{Results on \dl{} with \genQ{}}

Across both years of \dl{} we find that our FLAN-T5-EXAM approach supports the conclusions discussed above. 

We find that the \examqrels{} method correlates exceptionally well with the official leaderboard, obtaining spearman rank correlations of 0.93 in \dlfirst{} and 0.96 on \dlsecond{}, and kendall $\tau$ correlation of 0.8 and 0.84 respectively.  This is slightly better than the relevance-labeling prompt \texttt{Thom} \citep{thomas2023large} and slightlyworse than the prompt \texttt{Sun} \citep{sun2023chatgpt}.

The \examcover{} method correlates slightly less. This is likely because the \examcover{} focuses on coverage more than precision.

As mentioned before, a high inter-annotator agreement is not necessary for good leaderboard correlation. Nevertheless, our EXAM approach obtains an inter-annotator agreement score (Cohen's $\kappa$) that is in the range of relevance-prompting methods.


% * This result generalizes to other test collections such as DL19 and DL20, where the exam-qrels approach works slightly better than exam-cover.  Here our version of exam also performs similarly to approaches that directly ask to assess the relevance (e.g. Sun)
   %  - DL19  with inter-annotator agreement of kappa 0.36 , leaderboard correlation of  spearman 0.93, kenfall 0.8)  
   %   - this is in  in the ball park of Sun's prompts   (Kappa = 0.39, spearman - 0.96, kendall 0.85)
   % - DL20 :  kappa of 0.25, spearman 0.96, kendall 0.84
   %  - this is in the ball park of Sun's prompts (kappa 0.24 / spearman 0.96 / kendall 0.88) 
   

\input{results/correlation-dl19-self-rating--min-answers-2}


% \subsection{Results on TREC DL 2020 with \genQ{}}
\input{results/correlation-dl20-self-rated-min-answer-2}
% Leaderboard correlation on TREC DL 2020


% \subsection{FLAN-T5 family members \ld{drop?}}
% \begin{itemize}
% \item flan-t5-small:   spearman 0.32, kendall 0.29
% \item flan-t5-large: spearman 0.87  kendall 0.69

% \end{itemize}


% min_rating=4 nExam:CorrelationStats(spearman_correlation=0.31532207009587254, kendall_correlation=0.29184818148727604)
% min_rating=4  exam:CorrelationStats(spearman_correlation=0.31532207009587254, kendall_correlation=0.29184818148727604)
 
 % \eject 
 
\subsection{A Worked Example} \label{sec:worked-example}

To illustrate how our FLAN-T5-EXAM method functions, we present a detailed example from the \car{} dataset for query\_id \texttt{tqa2:L\_0384}. The passage presented below was retrieved at rank 1 by the \texttt{dangnt-nlp} method and was assessed by TREC judges as 'MUST be mentioned'.
 

\input{worked-example}

The \tqa{} question \texttt{NDQ\_007535} ``Outer layer of the skin?'' was correctly answered as ``epidermis''. Under the self-rating prompt, FLAN-T5 responds that question can be answered in a mostly relevant way but may have minor gaps (rating 4). 

A generated exam questions, ``How does the epidermis, dermis, and hypodermis work together to provide protection, sensation, and regulation for the body?'', also lead to a rating of 4.
While we cannot automatically confirm the correctness without an answer key, we manually highlight the relevant text spans in the passage.
%
To incorporate a human-in-the-loop, one would ask FLAN-T5 to produce an answer for the generated question, to be highlighted in a verification interface.


\input{results/dl19-leaderboard-correlation}
\input{results/dl20-leaderboard-correlation}


==> experimental-setup.tex <==
\subsection{Experimental Setup}

We study our approach in three experiments.

\begin{description}
\item[\car{} / \tqa{}:] Replicating the experimental setup of Sander et al by using queries and systems from \car{} \citep{dietz2019trec} which we evaluate with exam questions from the \tqa{} dataset \citep{Kembhavi2017TQA}.
\item[\car{} / \genQ{}:] Switching to our prompt-based generated question banks, we demonstrate that similar results are obtained when systems from \car{} are evaluated with a new set of generated questions.
\item[\dl{} 2019 \& 2020 / \genQ{}:] To demonstrate generalization to other datasets we use queries and systems from two years of \dl{} \citep{dl19,dl20} using a generated question bank for each test collection.
\end{description}

\noindent For all four experiments we use rankings of systems submitted to the respective TREC track (test data set) along with manually produced official TREC judgments.

The goals for the evaluation metric are:
\begin{description}
    \item[Leaderboard rank-correlation:] The leaderboard of systems under the \examcover{} and \examqrels{} metric should be similar to the official leaderboard. This is evaluated with two rank correlation measures: Spearman's rank correlation coefficient, measures differences in the leaderboard rank,  and Kendall's $\tau$ rank correlation which penalizes swaps of two systems on the leaderboard.
    \item[Inter-annotator agreement:] High passage-level agreement between official judgments and our predicted relevance labels. We provide count statistics and Cohen's $\kappa$ inter-annotator agreement which corrects for leniency vs strictness.
\end{description}

For question generation we use \texttt{gpt-3.5-turbo-instruct}; for question verification and self-rating we use \texttt{google/flan-t5-large} with the \texttt{text2text-generation} pipeline from Hugging Face.\footnote{\url{https://huggingface.co/google/flan-t5-large}} We also explored fine-tuning the FLAN-T5-large on the \squad{} dataset, but results were slightly worse.


We obtain ten questions for each of the 721 query-subtopics in \car{}, and each query in \dl{}.
%
We graded all passages in official judgments and the top 20 of all run submissions with EXAM. Across 131 queries in \car{} we grade, 85,329 passages. Across 43 queries in \dlfirst{}, we grade 9,260 passages. Across 54 queries in \dlsecond{}, we grade 11,386 passages. 
 
In \examqrels{} we use \treceval{}'s  \texttt{Precision@20} metric for simplicity. For self-rated approaches, we define a minimum rating of 4 as relevant (``strict'' binary relevance scale) unless otherwise specified.

\textbf{Baselines.}
We demonstrate that our approach is outperforming the original EXAM Answerability Metric \citep{sander2021exam}. Since Sander's work demonstrated that ROUGE metrics are uncorrelated with leaderboard rankings, we omit the comparison here.

Although prompt-based relevance judgments differ significantly in spirit from out approach, we provide several baselines as upper-bound reference  for the \dl{} experiments: \texttt{Sun} \citep{sun2023chatgpt}, \texttt{Fag}  \citep{faggioli2023perspectives}, \texttt{Thom}  (abridged prompt, grade 1 or better counted as relevant) \cite{thomas2023large}. Each prompt is used to directly grade passages for relevance with FLAN-T5-Large. We also explored suggested few-shot prompts but found that all of them lead to a drastically decreased quality---for example, for \texttt{Sun} a Spearman correlation of 0.4 instead of 0.96, and Kendall's $\tau$ of -0.01 instead of 0.24.

\textbf{Significance testing.} We perform a standard-error bar overlap test on all results and only describe significant improvements in the text. The standard error in all experiments ranges between 0.01 and 0.015. For brevity they are omitted here, but are available in the online appendix and illustrated in \ref{fig:car-y3-leaderboard}.

% \ld{move to intro}
% Soft goals:
% \begin{itemize}
%     \item Evaluation method that contributes to a reusable test collection that is repeatable and without biases to systems that did not contribute to the assessment pool. 
%     \item Fully-automatic evaluation method, that permits human verification and intervention.
%     \item Evaluation method that can be extended to improve coverage in areas that were missed.
%     \item Evaluation method that can compare retrieved content, generated content, and retrieval-augmented generated content.
% \end{itemize}

% Hard goals:
% \begin{itemize}
%     \item Evaluation metric that produces leaderboards that are similar to the official leaderboards of the track (but for less manual work)
%     \item (Less critical) Produces relevance labels that have a high inter-annotator agreement with manual judgments.
%     \item (Less critical) Easy integration into existing evaluation software, such as \treceval. 
% \end{itemize}



==> omitted/approach-exam-grading-with-flan-qa-system.tex <==
%% this text was omitted from this paper. We save it for a repro paper.

\subsubsection{Pre-processing System Responses}

To prepare the system responses for the grading phase, we break longer responses into paragraph-sized passages of roughly 400 tokens. For submitted passage rankings each passage will be considered individually. For each passage we obtain its plain text content and assign a unique \texttt{passage\_id}.

\subsubsection{EXAM Grading with Answer Checking} \label{sec:exam-grading-answer-verification}

To take advantage of the latest development in LLMs, 
%To make it easier to apply the EXAM Answerability Metric to new test collections, 
we propose to use an LLM-based \questionanswering{} system. While any LLM could be used, in this work we experiment with the FLAN-T5 family that became recently available. In particular we focus on the FLAN-T5-large model which can be run at reasonable speed on an NVIDIA A40 GPU.


Initially we used a simple prompt such as "context: \$passage; question: \$question".
As a technicality, the FLAN-T5 family only accepts prompts of up to 512 tokens. Should our \questionanswering{} prompt exceed this boundary, we truncate the given passage context to ensure that the question fits in the token allowance.

Unfortunately, modern LLM-based \questionanswering{} systems tend to answer questions from their memory rather than the given context. This is mitigated by (1) omitting the question choices from the prompt given to the LLM and (2) instructing the LLM in the prompt to ``provide a complete and concise answer to the question based on the context. ''


\paragraph{Fine-tuning for Unanswerable Questions}
For a \questionanswering{} system to be useful for our purposes, we would prefer an LLM that leaves a question unanswered when the provided passage context does not contain pertinent information.

\ld{check the spelling of SQUAD}
The SQUAD v2.0 is a suitable dataset to fine-tune an LLM for this purpose. The SQUAD v1.0 which provides contexts and questions, is extended in SQUAD v2.0 include more questions that are unanswerable with the given context. Hence in addition to an out-of-the-box version of FLAN-T5-large, we experiment with an version that is fine-tuned on the SQUAD v2.0 dataset to leave unanswerable questions unanswered. As discussed later, this reduces the set of questions that were answered correctly by memory.


\paragraph{Answer verification.}
By omitting the answer choices, the answer verification check is more involved as slight linguistic variations need to be handled. In our experiment we stem both the predicted and the gold answer, then count an answer as correct based on a Levenshtein distance of 0.8 or above.


% \begin{figure}
% \caption{Answer verification prompt. 
%      \label{fig:answer-verification-prompt}}
% \end{figure}

Since many correct answers are missed, we alternatively, use a FLAN-T5-large LLM to match given answer matches the correct answers. We use the following prompt:

\begin{quote}
     For the question "\{question\}" the correct answer is "\{correct\_answer\}". Is "\{answer\}" an equally correct response to this question? Answer yes or no.
\end{quote}
     
     
To give an example from exam question \texttt{L\_0016/NDQ\_000615} ``During very wet times, the water table will...'' for which the correct answer is ``rise'', this identifies additional answers including ``increase'', ``rising'', ``be higher'', ``increase substantially'' as well as ``During very wet times, the water table will rise.''

\paragraph{Checking for Unanswerability.} \label{sec:checking-unanswerability}
Given the technical difficulties to reliably verifying the correctness of answers, we propose an approach that scans the answer for expressions that the question is unanswerable with the provided context. 

In this variation, we count all answers as correct, except when they contain an invalid answer (such as ``a.'' or ``(iii)'') or one of the following expressions: 
"unanswerable"
,"no"
,"no answer",
"not enough information"
,"unknown"
,"it is not possible to tell"
,"it does not say"
, or "no relevant information".
 

==> omitted/approach-normalized-exam.tex <==

\paragraph{nEXAM.} 
Since it is possible that some exam questions are are phrased in a way that the \questionanswering{} system is unable to function (at no fault of the system), Sander suggests to empirically test which questions are answerable on a gold response. Since gold responses are usually not available for IR test collections, we propose to instead normalize 
with the set questions that are answerable with any system response.



==> omitted/discussion.tex <==
\section{Discussion}


\ld{move to discussion}
\begin{itemize}
    \item \textbf{Is this an open-book or closed-book exam?} Neither! The evaluated system is not even aware that it is put to the test and does not get to see the exam questions.
    \item \textbf{Isn't it unfair to judge a system by questions it does not know?} The system is asked to produce a relevant answer for the query, the exam questions are designed so that they verify important factoids that must be contained in order for the system response to be relevant.
    \item \textbf{Wouldn't the \examcover{} metric be affected by the quality of the internal question-answering system?} Yes, but there are several ways to verify that the quality of the Q/A system is sufficient: 
        \begin{enumerate}
            \item By manually inspecting extracted answers and comparing them to a gold answer key;
            \item by measuring the inter-annotator agreement with manual relevance judgments; 
            \item by confirming that the leaderboards agree with manual evaluation metrics.
        \end{enumerate}
\end{itemize}





==> omitted/related-work--other.tex <==


--
A wide range of approaches integrate passages, questions, and LLMs in some form.

Several approaches \citep{sachan2022improving,li2023llatrieval} aim to improve \questionanswering{} performance by using  retrieval-augmentation.


\citet{weng2023large} improve the LLM's reasoning ability by appending a backward verification step where answers are generated to be automatically answered by the LLM. \citeauthor{weng2023large} find that LLMs possess useful self-verification abilities, a result that we will build on in Section \ref{sec:exam-grading-self-rating}.

\citet{zhang2023towards} focus on fact verification, by breaking each claim down into several questions relevant to its factuality.

HELM \cite{liang2022holistic} evaluates the quality of an LLM via multiple tests. While this falls into a larger category of LLM-evaluation methods \cite{chang2023survey} (out of scope),  \ld{check tense} one of its test is asking for determining the relevance of a passage. We will use this prompt in our evaluation.




==> omitted/related-work--semantic-matching.tex <==

\bigskip
\ld{ --- Maybe end related work here ---}
\subsection{Semantic Text Matching}
    Any approach that uses questions with free-form answers, matches nuggets, or directly compares retrieved passages to known relevant responses relies on some form of semantic text matching.

    ROUGE, METEOR \ld{cite}, as well as nugget-based evaluation \cite{pavlu2012ir} focus on word (or ngram) overlap matches  ("shingles"). However, because relevant information can be rephrased using different words, an exact match of words is not necessary for being relevant. Polysemy can lead to false matches.

    BertScore \ld{cite} and Word Mover Distance \ld{is this really using embeddings?} use contextual word embeddings for the matching decision, thereby addressing the issue of synonyms and polysemy. \ld{drop? Variants differ in matching bags of tokens, sequences of tokens, or embeddings of the whole text.}
    These approaches work well on short and concise texts, but deteriorate in quality as the texts get longer. The approach breaks down when are written in different linguistic styles, e.g., social media vs.\ textbook.

    In this work, instead of sequences of words, we focus on matching relevant information content: We acknowledge that different pieces of relevant information (akin to nuggets) can be scattered throughout the system response in no particular order. Each piece of information can be expressed in a complex way, and hence is ``matched'' by answering a question in a concise manner. \ld{drop?  When this answer will be verified for correctness against an answer key, where we have to resort to some form to text matching. Nevertheless, such answers are short and concise text spans, where many of the matching approaches above are known to work reliably.}


==> omitted/related-work-test-questions-exam.tex <==

The original EXAM method relies solely on humans to design the exam, with the intent that only a human could identify the core questions that would need to be addressed in a relevant answer. This is in contrast to approaches that generate questions from a gold summary (detailed in Section \ref{sec:rw-test-questions}), which might lead to questions derived from non-relevant aspects mentioned in relevant text.
In contrast, our approach directly generated an initial set of query-relevant questions via a generative LLM (such as chatGPT \cite{chatgpt}). 


==> omitted/result--car-tqa-qa-squad2-cc.tex <==

\textcolor{purple}{After meditating on numbers, I decided to focus on the nltk-based answer verification with the CC prompt, as this gives the highest leaderboard correlation.  The other experiments can go in a reproduction paper, including this text below:}

In our first experiment, we use the exam question banks from the TQA dataset. Each question comes with a human-designed gold answer. As part of the exam grading, we ask the LLM to answer each exam question with each passage from the system response, then verify the predicted answer with the gold answer. 

The answer verification is performed by a heuristic that uses string normalization, stemming, and levenshtein distance as well as special handling for true/false questions. 

We compare three setups for question answering:
\begin{description}
    \item[QA] Standard Q/A prompt on out-of-the box FLAN-T5-large using the text2text pipeline with a simple prompt ``Context: {context}; Question: {question}''. The concern is that the LLM will answer the question correctly from memory rather than the provided context.
    \item[CC] Out-of-the-box FLAN-T5-large with a prompt that instructs to ``provide a complete and concise answer to the question based on the context. Question: {question} Context: {context}.''
    \item[Squad2] A Squad2-finetuned FLAN-T5-large following the mandated format of context and question.
\end{description}


The resulting \examcover{} leaderboard produced with each approach has a reasonable correlation with the official CAR-Y3 leaderboard as displayed in Table \ref{tab:qa-leaderboard-correlation}, with  \method{CC} approach being clearly the best.

\begin{table}[h]
\caption{Rank-correlation with the official \car{} leaderboard of system rankings using \questionanswering with answer verification. \label{tab:qa-leaderboard-correlation}}

% nltk
\begin{tabular}{ccc}
 & spearman & kendall\tabularnewline
CC & 0.94 & 0.84\tabularnewline
QA & 0.82 & 0.67\tabularnewline
Squad2 & 0.84 & 0.69\tabularnewline
\end{tabular}

% v5
% \begin{tabular}{ccc}
%  & spearman & kendall\tabularnewline
% CC & 0.88 & 0.72\tabularnewline
% QA & 0.72 & 0.53\tabularnewline
% Squad2 & 0.86 & 0.74\tabularnewline
% \end{tabular}
\end{table}


Because of the very different evaluation paradigm, we do not expect a high inter-annotator agreement of our automatic relevance labeling vs manual TREC judges and indeed, the per-passage inter-annotator agreement is very low ($\kappa \approx 0.07$) across all three approaches. 

Of the 6352 questions, \method{QA} answers the higher number of questions correctly (3519), followed by \method{CC} (1005). In both cases, half the questions are associated with negatively judged passages. \method{Squad2} is able to correctly answer only 409 questions, while two-thirds are associated with a relevant passage judgments, too few positive responses (6\%)  render the approach not useful for our purposes.



----

Of the 6352 questions, \method{QA} answers the higher number of questions correctly (3519), followed by \method{CC} (1005). In both cases, half the questions are associated with negatively judged passages. \method{Squad2} is able to correctly answer only 409 questions, while two-thirds are associated with a relevant passage judgments, too few positive responses (6\%)  render the approach not useful for our purposes.

==> prompt-table.tex <==
\begin{table*}[ht]
    \caption{ Question generation prompts (\genQ{}). \label{tab:prompt-table}}

\begin{tabular}{p{0.45\linewidth} p{0.45\linewidth} }
    \toprule
    \textbf {Question Generation: TREC DL Prompt} & \textbf{Question Generation: TREC CAR Y3 Prompt} \\
    % \midrule
    
     Break the query '\{query\_title\}' into concise questions that must be answered. Generate 10 concise insightful questions that reveal whether information relevant for '\{query\_title\}' was provided, showcasing a deep understanding of the subject matter. Avoid basic or introductory-level inquiries. Keep the questions short and in a Python list format. & Explore the connection between '\{query\_title\}' with a specific focus on the subtopic '\{query\_subtopic\}'. Generate insightful questions that delve into advanced aspects of '\{query\_subtopic\}', showcasing a deep understanding of the subject matter. Avoid basic or introductory-level inquiries. Give the question set in a Python list format.\\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{table}[h]
    \caption{ Grading prompts. \label{tab:qa-prompt-table}}

\begin{tabular}{p{0.95\linewidth} }
    \toprule
    \textbf {Grading: Question Answering Prompt}  \tabularnewline
    % \midrule
    % \makecell{
    \parbox[t]{0.95\linewidth}{
    provide a complete and concise answer to the question based on the context.
    Question: \{question\}
    Context: \{context\} 
    }\tabularnewline
    \midrule
    % \medskip
    \textbf {Grading: Self-rating Prompt}  \tabularnewline
    % \midrule
    % \makecell{
    \parbox[t]{0.95\linewidth}{
Can the question be answered based on the available 
context? choose one: \\
- 5: The answer is highly relevant, complete, and 
accurate.\\
- 4: The answer is mostly relevant and complete but may
have minor gaps or inaccuracies.\\
- 3: The answer is partially relevant and complete, with 
noticeable gaps or inaccuracies.\\
- 2: The answer has limited relevance and completeness, 
with significant gaps or inaccuracies.\\
- 1: The answer is minimally relevant or complete, with 
substantial shortcomings.\\
- 0: The answer is not relevant or complete at all. \\
Question: \{question\}
Context: \{context\} 
}\tabularnewline
    \bottomrule
  \end{tabular}
\end{table}



==> results/car-y3-leaderboard-correlation.tex <==
% Preview source code for paragraph 0
\begin{small}

% Preview source code for paragraph 0

\begin{tabular}{lccccc}
\toprule
CAR-Y3 & \makecell{TQA \\ EXAM \\ Cover} & \makecell{GenQ \\  EXAM \\ Cover} & \makecell{GenQ \\ EXAM \\ Qrels} & \makecell{official \\ rank \\ } & \makecell{TQA \\ \citep{sander2021exam} \\ rank}  \tabularnewline
%method && & & & \tabularnewline
% method & \begin{sideways}ExamCover\end{sideways} & \begin{sideways}ExamCover\end{sideways} & \begin{sideways}ExamQrels\end{sideways} & \begin{sideways}rank\end{sideways} & \begin{sideways}rank\end{sideways}\tabularnewline
\midrule 
\_overall\_ & 0.388 & 0.811 & 1 &  & \tabularnewline
dangnt-nlp & 0.300 & 0.609 & 0.555 & 1 & 2\tabularnewline
ReRnak3\_BERT & 0.288 & 0.620 & 0.594 & 2 & 5\tabularnewline
ECNU\_ReRank1 & 0.285 & 0.572 & 0.512 & 8 & 12\tabularnewline
ReRnak2\_BERT & 0.281 & 0.623 & 0.593 & 3 & 1\tabularnewline
IRIT1 & 0.279 & 0.569 & 0.540 & 5 & 7\tabularnewline
IRIT2 & 0.279 & 0.569 & 0.540 & 5 & 4\tabularnewline
IRIT3 & 0.279 & 0.569 & 0.540 & 5 & 9\tabularnewline
ECNU\_BM25 & 0.278 & 0.604 & 0.588 &  & \tabularnewline
ECNU\_BM25\_1 & 0.278 & 0.602 & 0.586 & 8 & 11\tabularnewline
ICT-BM25 & 0.278 & 0.598 & 0.576 &  & \tabularnewline
Bert-ConvKNRM-50 & 0.277 & 0.605 & 0.571 & 9 & 6\tabularnewline
UNH-bm25-rm & 0.276 & 0.545 & 0.535 &  & \tabularnewline
bm25-populated & 0.275 & 0.547 & 0.502 & 10 & 8\tabularnewline
UNH-qee & 0.271 & 0.614 & 0.568 &  & \tabularnewline
UNH-bm25-ecmpsg & 0.267 & 0.522 & 0.487 & 11 & 10\tabularnewline
Bert-ConvKNRM & 0.248 & 0.503 & 0.395 &  & \tabularnewline
Bert-DRMMTKS & 0.247 & 0.366 & 0.251 & 12 & 3\tabularnewline
ICT-DRMMTKS & 0.237 & 0.369 & 0.247 & 16 & 13\tabularnewline
UvABottomUp2 & 0.148 & 0.251 & 0.289 & 15 & 16\tabularnewline
UvABM25RM3 & 0.147 & 0.260 & 0.300 & 13 & 15\tabularnewline
UvABottomUpCh. & 0.145 & 0.255 & 0.283 & 14 & 14\tabularnewline
UvABottomUp1 & 0.142 & 0.209 & 0.233 &  & \tabularnewline
\midrule 
spearman & 0.937 & 0.869 & 0.865 &  & 0.75\tabularnewline
kendall & 0.841 & 0.687 & 0.738 &  & 0.57\tabularnewline
\bottomrule
\end{tabular}
\end{small}




==> results/correlation--car-tqa-cc-corrected.tex <==

% \normalsize%
% \section{correlation tables}%
% \label{sec:correlationtables}%
 

% %
% \section{min answers 1}%
% \label{sec:minanswers1}%
 

%

\begin{table}[]
\caption{Inter-annotator agreement on \car{} / \tqa{} question banks using \questionanswering{} with answer verification. Boxed cells indicate mappings from label to judgment. Largest count per column is depicted in bold.
%min answer = 1
\label{tab:car-tqa-binary-cohen}}
\begin{tabu}{@{}llcclr@{}}%
\toprule%
\multirow{4}{*}{\begin{sideways}BINARY\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
\cmidrule(l@{\tabcolsep}){3-4}%
&&1+2+3&0&&\\%
\cmidrule(l@{\tabcolsep}){1-6}%
&1&\fbox{{553}}&452&1005&0.078\\%
&0&\textbf{2237}&\fbox{\textbf{3110}}&5347&0.079\\\bottomrule%
\end{tabu}%
\end{table}

% \par%
% \begin{tabu}{@{}llcccclr@{}}%
% \toprule%
% \multirow{4}{*}{\begin{sideways}GRADED\end{sideways}}&\textbf{Label}&\multicolumn{4}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-6}%
% &&3&2&1&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-8}%
% &1&111&\fbox{328}&114&\textbf{452}&1005&0.077\\%
% &0&409&1249&579&\fbox{\textbf{3110}}&5347&0.079\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \section{min answers 2}%
% \label{sec:minanswers2}%
 

% %
% \begin{tabu}{@{}llcclr@{}}%
% \toprule%
% \multirow{4}{*}{\begin{sideways}BINARY\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-4}%
% &&1+2+3&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-6}%
% &1&\fbox{\textbf{223}}&134&357&0.047\\%
% &0&2567&\fbox{\textbf{3428}}&5995&0.049\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \begin{tabu}{@{}llcccclr@{}}%
% \toprule%
% \multirow{4}{*}{\begin{sideways}GRADED\end{sideways}}&\textbf{Label}&\multicolumn{4}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-6}%
% &&3&2&1&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-8}%
% &1&43&\fbox{\textbf{138}}&42&134&357&0.057\\%
% &0&477&1439&651&\fbox{\textbf{3428}}&5995&0.049\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \section{min answers 5}%
% \label{sec:minanswers5}%
 

% %
% \begin{tabu}{@{}llcclr@{}}%
% \toprule%
% \multirow{4}{*}{\begin{sideways}BINARY\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-4}%
% &&1+2+3&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-6}%
% &1&\fbox{\textbf{4}}&2&6&0.00093\\%
% &0&2786&\fbox{\textbf{3560}}&6346&0.0011\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \begin{tabu}{@{}llcccclr@{}}%
% \toprule%
% \multirow{4}{*}{\begin{sideways}GRADED\end{sideways}}&\textbf{Label}&\multicolumn{4}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-6}%
% &&3&2&1&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-8}%
% &1&0&\fbox{\textbf{4}}&0&2&6&0.0031\\%
% &0&520&1573&693&\fbox{\textbf{3560}}&6346&0.0011\\\bottomrule%
% %
% \end{tabu}%
% \par%


==> results/correlation-car-naghmeh-self-rating.tex <==
% \normalsize%
% \section{correlation tables}%
% \label{sec:correlationtables}%
 

% %
% \section{Min Answers= 1}%
% \label{sec:MinAnswers=1}%
 

% %
% \begin{tabu}{@{}llcccclr@{}}%
% \toprule%
% \multirow{8}{*}{\begin{sideways}GRADED\end{sideways}}&\textbf{Label}&\multicolumn{4}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-6}%
% &&3&2&1&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-8}%
% &5&51&\fbox{\textbf{164}}&56&130&401&0.073\\%
% &4&431&\fbox{1223}&540&\textbf{2059}&4253&0.094\\%
% &3&2&16&\fbox{7}&\textbf{67}&92&{-}0.008\\%
% &2&14&44&\fbox{13}&\textbf{122}&193&{-}0.02\\%
% &1&0&24&\fbox{17}&\textbf{141}&182&{-}0.0074\\%
% &0&22&106&60&\fbox{\textbf{1043}}&1231&0.21\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \begin{tabu}{@{}llccclr@{}}%
% \toprule%
% \multirow{5}{*}{\begin{sideways}MERGE\end{sideways}}&\textbf{Label}&\multicolumn{3}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-5}%
% &&2+3&1&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-7}%
% &4+5&\fbox{1869}&596&\textbf{2189}&4654&0.19\\%
% &1+2+3&100&\fbox{37}&\textbf{330}&467&{-}0.028\\%
% &0&128&60&\fbox{\textbf{1043}}&1231&0.21\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \begin{tabu}{@{}llcclr@{}}%
% \toprule%
% \multirow{4}{*}{\begin{sideways}LENIENT\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-4}%
% &&1+2+3&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-6}%
% &1+2+3+4+5&\fbox{\textbf{2602}}&2519&5121&0.22\\%
% &0&188&\fbox{\textbf{1043}}&1231&0.21\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \begin{tabu}{@{}llcclr@{}}%
% \toprule%
% \multirow{4}{*}{\begin{sideways}STRICT\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-4}%
% &&1+2+3&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-6}%
% &4+5&\fbox{\textbf{2465}}&2189&4654&0.26\\%
% &0+1+2+3&325&\fbox{\textbf{1373}}&1698&0.25\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \section{Min Answers= 2}%
% \label{sec:MinAnswers=2}%
 
\begin{table}[]
\caption{Inter-annotator agreement on \car{} / \genQ{} question banks using self-ratings. Top: Graded ratings-vs-judgments. Rating 4 is most frequently associated with a positive grade. Middle: Lenient relevance for ratings $\geq 1$. Bottom: Strict relevance when ratings  $\geq 4$. %Boxed cells indicate mappings from label to judgment. Largest count per column is depicted in bold.
%min answer = 2
\label{tab:car-genq-cohen}}
%
\begin{tabu}{@{}llccccr}%
\toprule%
\multirow{8}{*}{\begin{sideways}GRADED\end{sideways}}&\textbf{Label}&\multicolumn{4}{c}{\textbf{Judgments}}&\textbf{Total}\\%
\cmidrule(l@{\tabcolsep}){3-6}%
&&3&2&1&0&\\%
\cmidrule(l@{\tabcolsep}){1-7}%
&5&11&\fbox{{52}}&13&20&96\\%
&4&\textbf{430}&\fbox{\textbf{1121}}&\textbf{472}&{1425}&3448\\%
&3&5&33&\fbox{19}&{98}&155\\%
&2&17&76&\fbox{27}&{217}&337\\%
&1&5&57&\fbox{23}&{160}&245\\%
&0&52&238&139&\fbox{\textbf{1642}}&2071\\\bottomrule%
%
\end{tabu}%

%with kappa!
% \begin{tabu}{@{}llcccclr@{}}%
% \toprule%
% \multirow{8}{*}{\begin{sideways}GRADED\end{sideways}}&\textbf{Label}&\multicolumn{4}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-6}%
% &&3&2&1&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-8}%
% &5&11&\fbox{{52}}&13&20&96&0.034\\%
% &4&\textbf{430}&\fbox{\textbf{1121}}&\textbf{472}&{1425}&3448&0.17\\%
% &3&5&33&\fbox{19}&{98}&155&0.0059\\%
% &2&17&76&\fbox{27}&{217}&337&{-}0.021\\%
% &1&5&57&\fbox{23}&{160}&245&{-}0.0081\\%
% &0&52&238&139&\fbox{\textbf{1642}}&2071&0.29\\\bottomrule%
% %
% \end{tabu}%


\par%
% \begin{tabu}{@{}llccclr@{}}%
% \toprule%
% \multirow{5}{*}{\begin{sideways}MERGE\end{sideways}}&\textbf{Label}&\multicolumn{3}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-5}%
% &&2+3&1&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-7}%
% &4+5&\fbox{\textbf{1614}}&485&1445&3544&0.28\\%
% &1+2+3&193&\fbox{69}&\textbf{475}&737&{-}0.017\\%
% &0&290&139&\fbox{\textbf{1642}}&2071&0.29\\\bottomrule%
% %
% \end{tabu}%
% \par%


\begin{tabu}{@{}llcclr@{}}%
\toprule%
\multirow{4}{*}{\begin{sideways}LENIENT\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
\cmidrule(l@{\tabcolsep}){3-4}%
&&1+2+3&0&&\\%
\cmidrule(l@{\tabcolsep}){1-6}%
&1+2+3+4+5&\fbox{\textbf{2361}}&1920&4281&0.3\\%
&0&429&\fbox{\textbf{1642}}&2071&0.29\\\bottomrule%
%
\end{tabu}%
\par%
\begin{tabu}{@{}llcclr@{}}%
\toprule%
\multirow{4}{*}{\begin{sideways}STRICT\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
\cmidrule(l@{\tabcolsep}){3-4}%
&&1+2+3&0&&\\%
\cmidrule(l@{\tabcolsep}){1-6}%
&4+5&\fbox{\textbf{2099}}&1445&3544&0.35\\%
&0+1+2+3&691&\fbox{\textbf{2117}}&2808&0.34\\\bottomrule%
%
\end{tabu}%
\end{table}

% \par%
% \section{Min Answers= 5}%
% \label{sec:MinAnswers=5}%
 

% %
% \begin{tabu}{@{}llcccclr@{}}%
% \toprule%
% \multirow{8}{*}{\begin{sideways}GRADED\end{sideways}}&\textbf{Label}&\multicolumn{4}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-6}%
% &&3&2&1&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-8}%
% &5&0&\fbox{\textbf{6}}&0&0&6&0.0057\\%
% &4&284&\fbox{\textbf{650}}&249&541&1724&0.18\\%
% &3&6&45&\fbox{34}&\textbf{93}&178&0.037\\%
% &2&27&103&\fbox{43}&\textbf{208}&381&0.003\\%
% &1&11&93&\fbox{33}&\textbf{128}&265&0.01\\%
% &0&192&680&334&\fbox{\textbf{2592}}&3798&0.3\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \begin{tabu}{@{}llccclr@{}}%
% \toprule%
% \multirow{5}{*}{\begin{sideways}MERGE\end{sideways}}&\textbf{Label}&\multicolumn{3}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-5}%
% &&2+3&1&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-7}%
% &4+5&\fbox{\textbf{940}}&249&541&1730&0.28\\%
% &1+2+3&285&\fbox{110}&\textbf{429}&824&0.032\\%
% &0&872&334&\fbox{\textbf{2592}}&3798&0.3\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \begin{tabu}{@{}llcclr@{}}%
% \toprule%
% \multirow{4}{*}{\begin{sideways}LENIENT\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-4}%
% &&1+2+3&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-6}%
% &1+2+3+4+5&\fbox{\textbf{1584}}&970&2554&0.31\\%
% &0&1206&\fbox{\textbf{2592}}&3798&0.3\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \begin{tabu}{@{}llcclr@{}}%
% \toprule%
% \multirow{4}{*}{\begin{sideways}STRICT\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-4}%
% &&1+2+3&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-6}%
% &4+5&\fbox{\textbf{1189}}&541&1730&0.29\\%
% &0+1+2+3&1601&\fbox{\textbf{3021}}&4622&0.3\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \end{document}

==> results/correlation-dl19-self-rating--min-answers-2.tex <==
% \par%
% \section{Min Answers= 2}%
% \label{sec:MinAnswers=2}%
 
% { \color{lightgray}
% %
% \begin{tabu}{@{}llcccclr@{}}%
% \toprule%
% \multirow{8}{*}{\begin{sideways}GRADED\end{sideways}}&\textbf{Label}&\multicolumn{4}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-6}%
% &&3&2&1&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-8}%
% &5&\fbox{88}&\textbf{100}&38&65&291&0.14\\%
% &4&\fbox{255}&\textbf{996}&543&710&2504&0.047\\%
% &3&27&\fbox{61}&80&\textbf{161}&329&{-}0.0031\\%
% &2&6&\fbox{82}&66&\textbf{113}&267&0.03\\%
% &1&5&\fbox{7}&10&\textbf{23}&45&{-}0.0019\\%
% &0&316&558&864&\fbox{\textbf{4086}}&5824&0.37\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \begin{tabu}{@{}llccclr@{}}%
% \toprule%
% \multirow{5}{*}{\begin{sideways}MERGE\end{sideways}}&\textbf{Label}&\multicolumn{3}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-5}%
% &&3&2&0+1&&\\%
% \cmidrule(l@{\tabcolsep}){1-7}%
% &4+5&\fbox{343}&1096&\textbf{1356}&2795&0.086\\%
% &1+2+3&38&\fbox{150}&\textbf{453}&641&0.023\\%
% &0&316&558&\fbox{\textbf{4950}}&5824&0.34\\\bottomrule%
% %
% \end{tabu}%
% }
% \par%


\begin{table}[]
\caption{Inter-annotator agreement on \dlfirst{} / \genQ{} question banks using self-ratings.  Top: Lenient relevance. Bottom: Strict relevance.
%min answer = 2
\label{tab:dl19-genq-cohen}}
\begin{tabu}{@{}llcclr@{}}%
\toprule%
\multirow{4}{*}{\begin{sideways}LENIENT\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
\cmidrule(l@{\tabcolsep}){3-4}%
&&2+3&0+1&&\\%
\cmidrule(l@{\tabcolsep}){1-6}%
&1+2+3+4+5&\fbox{\textbf{1627}}&{1809}&3436&0.34\\%
&0&874&\fbox{\textbf{4950}}&5824&0.34\\\bottomrule%
%
\end{tabu}%
\par%
\begin{tabu}{@{}llcclr@{}}%
\toprule%
\multirow{4}{*}{\begin{sideways}STRICT\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
\cmidrule(l@{\tabcolsep}){3-4}%
&&2+3&0+1&&\\%
\cmidrule(l@{\tabcolsep}){1-6}%
&4+5&\fbox{\textbf{1439}}&1356&2795&0.36\\%
&0+1+2+3&1062&\fbox{\textbf{5403}}&6465&0.36\\\bottomrule%
%
\end{tabu}%

Comparison $\kappa$: \texttt{Sun} 0.39 / \texttt{Fag} 0.44 / \texttt{Thom} 0.08
\end{table}


==> results/correlation-dl20-self-rated-min-answer-2.tex <==
% \section{Min Answers= 2}%
% \label{sec:MinAnswers=2}%
 
% { \color{lightgray}
% %
% \begin{tabu}{@{}llcccclr@{}}%
% \toprule%
% \multirow{8}{*}{\begin{sideways}GRADED\end{sideways}}&\textbf{Label}&\multicolumn{4}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-6}%
% &&3&2&1&0&&\\%
% \cmidrule(l@{\tabcolsep}){1-8}%
% &5&\fbox{37}&70&54&\textbf{162}&323&0.04\\%
% &4&\fbox{368}&554&792&\textbf{1429}&3143&0.11\\%
% &3&37&\fbox{36}&98&\textbf{314}&485&{-}0.011\\%
% &2&21&\fbox{55}&106&\textbf{290}&472&0.018\\%
% &1&5&\fbox{20}&24&\textbf{44}&93&0.021\\%
% &0&178&285&866&\fbox{\textbf{5541}}&6870&0.32\\\bottomrule%
% %
% \end{tabu}%
% \par%
% \begin{tabu}{@{}llccclr@{}}%
% \toprule%
% \multirow{5}{*}{\begin{sideways}MERGE\end{sideways}}&\textbf{Label}&\multicolumn{3}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
% \cmidrule(l@{\tabcolsep}){3-5}%
% &&3&2&0+1&&\\%
% \cmidrule(l@{\tabcolsep}){1-7}%
% &4+5&\fbox{405}&624&\textbf{2437}&3466&0.11\\%
% &1+2+3&63&\fbox{111}&\textbf{876}&1050&0.018\\%
% &0&178&285&\fbox{\textbf{6407}}&6870&0.22\\\bottomrule%
% %
% \end{tabu}%
% }

% \par%

\begin{table}[]
\caption{Inter-annotator agreement on \dlsecond{} / \genQ{} question banks using self-ratings.  Top: Lenient relevance. Bottom: Strict relevance.
%min answer = 2
\label{tab:dl20-genq-cohen}}

\begin{tabu}{@{}llcclr@{}}%
\toprule%
\multirow{4}{*}{\begin{sideways}LENIENT\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
\cmidrule(l@{\tabcolsep}){3-4}%
&&2+3&0+1&&\\%
\cmidrule(l@{\tabcolsep}){1-6}%
&1+2+3+4+5&\fbox{\textbf{1203}}&{3313}&4516&0.22\\%
&0&463&\fbox{\textbf{6407}}&6870&0.22\\\bottomrule%
%
\end{tabu}%
\par%
\begin{tabu}{@{}llcclr@{}}%
\toprule%
\multirow{4}{*}{\begin{sideways}STRICT\end{sideways}}&\textbf{Label}&\multicolumn{2}{c}{\textbf{Judgments}}&\textbf{Total}&\textbf{Cohen's }$\boldsymbol{\kappa}$\\%
\cmidrule(l@{\tabcolsep}){3-4}%
&&2+3&0+1&&\\%
\cmidrule(l@{\tabcolsep}){1-6}%
&4+5&\fbox{\textbf{1029}}&{2437}&3466&0.25\\%
&0+1+2+3&637&\fbox{\textbf{7283}}&7920&0.25\\\bottomrule%
%
\end{tabu}%

Comparison $\kappa$: \texttt{Sun} 0.24 / \texttt{Fag} 0.29 / \texttt{Thom} 0.08
\end{table}
% \par%

==> results/dl19-leaderboard-correlation.tex <==
\begin{table}[b]
\caption{Leaderboard for \dlfirst{}, using ratings $\geq 3$ as relevant. 
%Some methods omitted to not violate page margins.
\label{tab:dl2019-leaderboard}}
\begin{tabular}{lllc}
\toprule
DL2019               & \makecell{EXAM\\Cover}  & \makecell{EXAM\\Qrels} & \makecell{Official \\ Rank} \\
% method               &   &   &  \\

\midrule
% \_overall\_          & 0.900   & 1.000          &                               \\
% TUW19-p3-f           & 0.726 & 0.7116          & 13                            \\
% srchvrs\_ps\_run3    & 0.716 & 0.6698          & 24                            \\
% TUW19-p2-f           & 0.714 & 0.7198          & 17                            \\
% TUW19-p1-f           & 0.716 & 0.7407          & 14                            \\
% srchvrs\_ps\_run2    & 0.712 & 0.7128          & 19                            \\
% idst\_bert\_p2       & 0.707 & 0.7593          & 2                             \\
% idst\_bert\_p3       & 0.707 & 0.7558          & 3                             \\
% idst\_bert\_p1       & 0.702 & 0.7523          & 1                             \\
% p\_exp\_bert         & 0.700   & 0.7442          & 8                             \\
% p\_exp\_rm3\_bert    & 0.700   & 0.7547          & 4                             \\
% TUW19-p2-re          & 0.695 & 0.7023          & 20                            \\
% runid3               & 0.695 & 0.7256          & 12                            \\
% idst\_bert\_pr2      & 0.695 & 0.7512          & 6                             \\
% p\_bert              & 0.695 & 0.7453          & 5                             \\
% ICT-CKNRM\_B50       & 0.693 & 0.6884          & 23                            \\
% ICT-CKNRM\_B         & 0.686 & 0.6349          & 21                            \\
% ICT-BERT2            & 0.686 & 0.6349          & 18                            \\
% runid4               & 0.691 & 0.7209          & 11                            \\
% TUW19-p3-re          & 0.688 & 0.7047          & 15                            \\
% idst\_bert\_pr1      & 0.688 & 0.7453          & 7                             \\
% srchvrs\_ps\_run1    & 0.681 & 0.6442          & 34                            \\
% TUW19-p1-re          & 0.686 & 0.7035          & 16                            \\
% ms\_duet\_passage    & 0.684 & 0.7395          & 22                            \\
% TUA1-1               & 0.684 & 0.5849          & 10                            \\
% test1                & 0.684 & 0.6174          & 9                             \\
% runid5               & 0.681 & 0.5860           & 30                            \\
% bm25base\_p          & 0.677 & 0.6791          & 33                            \\
% runid2               & 0.674 & 0.6849          & 29                            \\
% bm25base\_ax\_p      & 0.667 & 0.6174          & 26                            \\
% bm25tuned\_ax\_p     & 0.665 & 0.6512          & 27                            \\
% bm25tuned\_prf\_p    & 0.665 & 0.6593          & 25                            \\
% bm25tuned\_p         & 0.663 & 0.5837          & 35                            \\
% bm25base\_prf\_p     & 0.660  & 0.1453          & 28                            \\
\_overall\_       & 0.900   & 1      &    \\
idst\_bert\_p2    & 0.707 & 0.759 & 2    \\
idst\_bert\_p3    & 0.707 & 0.756 & 3    \\
p\_exp\_rm3\_bert & 0.700   & 0.755 & 4    \\
idst\_bert\_p1    & 0.702 & 0.752 & 1    \\
idst\_bert\_pr2   & 0.695 & 0.751 & 6    \\
p\_bert           & 0.695 & 0.745 & 5    \\
idst\_bert\_pr1   & 0.688 & 0.745 & 7    \\
p\_exp\_bert      & 0.700   & 0.744 & 8    \\
TUW19-p1-f        & 0.716 & 0.741 & 14   \\
ms\_duet\_passage & 0.684 & 0.740 & 22   \\
runid3            & 0.695 & 0.726 & 12   \\
runid4            & 0.691 & 0.721 & 11   \\
TUW19-p2-f        & 0.714 & 0.720 & 17   \\
srchvrs\_ps\_run2 & 0.712 & 0.713 & 19   \\
TUW19-p3-f        & 0.726 & 0.712 & 13   \\
TUW19-p3-re       & 0.688 & 0.705 & 15   \\
TUW19-p1-re       & 0.686 & 0.704 & 16   \\
TUW19-p2-re       & 0.695 & 0.702 & 20   \\
ICT-CKNRM\_B50    & 0.693 & 0.688 & 23   \\
runid2            & 0.674 & 0.685 & 29   \\
bm25base\_p       & 0.677 & 0.679 & 33   \\
srchvrs\_ps\_run3 & 0.716 & 0.670 & 24   \\
bm25tuned\_prf\_p & 0.665 & 0.659 & 25   \\
bm25tuned\_ax\_p  & 0.665 & 0.651 & 27   \\
srchvrs\_ps\_run1 & 0.681 & 0.644 & 34   \\
ICT-CKNRM\_B      & 0.686 & 0.635 & 21   \\
ICT-BERT2         & 0.686 & 0.635 & 18   \\
test1             & 0.684 & 0.617 & 9    \\
bm25base\_ax\_p   & 0.667 & 0.617 & 26   \\
runid5            & 0.681 & 0.586  & 30   \\
TUA1-1            & 0.684 & 0.585 & 10   \\
bm25tuned\_p      & 0.663 & 0.584 & 35   \\
bm25base\_prf\_p  & 0.660  & 0.145 & 28  \\
% bm25tuned\_rm3\_p    & 0.658 &                 & 31                            \\
% bm25base\_rm3\_p     & 0.658 &                 & 32                            \\
% UNH\_bm25            & 0.647 &                 & 36                            \\
% UNH\_exDL\_bm25      & 0.188 &                 &                               \\
\midrule
                     % &       &                 &                               \\
% min\_rating          & 3     & 3               &     Sun / FagB / HELM                          \\
  &     &          &       \texttt{Sun} / \texttt{Fag} / \texttt{Thom}                          \\
Spearman correlation & 0.72  & 0.93            &    0.96 / 0.96 / 0.86                           \\
Kendall correlation  & 0.54  & 0.80             &    0.85 / 0.85 / 0.67         \\
\bottomrule

\end{tabular}
\end{table}

==> results/dl20-leaderboard-correlation.tex <==
\begin{table}[]
\caption{Leaderboard for \dlsecond{}, using ratings $\geq 4$ as relevant. Some methods omitted to not violate page margins.\label{tab:dl2020-leaderboard}}
\begin{small}
\begin{tabular}{lllc}
\toprule
DL2020               & \makecell{EXAM\\Cover}  & \makecell{EXAM\\Qrels} & \makecell{Official \\ Rank} \\
% DL2020                & EXAM Cover  & EXAM Qrels & Official Rank \\
% method                &       & Evaluation & leaderboard \\
\midrule
\_overall\_          & 0.911 & 1.000 &    \\
NLE\_pr3             & 0.748 & 0.786 & 12 \\
pash\_f2             & 0.744 & 0.786 & 5  \\
pash\_f3             & 0.741 & 0.786 & 3  \\
pash\_f1             & 0.741 & 0.785 & 4  \\
NLE\_pr2             & 0.737 & 0.783 & 16 \\
CoRT-electra         & 0.731 & 0.781 & 9  \\
pash\_r3             & 0.739 & 0.778 & 1  \\
NLE\_pr1             & 0.743 & 0.777 & 17 \\
p\_d2q\_bm25\_duo    & 0.756 & 0.776 & 6  \\
pinganNLP2           & 0.741 & 0.776 & 13 \\
pinganNLP1           & 0.741 & 0.776 & 15 \\
pash\_r2             & 0.739 & 0.776 & 2  \\
RMIT-Bart            & 0.737 & 0.776 & 10 \\
pash\_r1             & 0.735 & 0.775 & 11 \\
p\_d2q\_rm3\_duo     & 0.752 & 0.773 & 7  \\
rr-pass-roberta      & 0.741 & 0.769 & 22 \\
pinganNLP3           & 0.741 & 0.769 & 14 \\
bigIR-T5-BERT-F      & 0.720 & 0.766 & 26 \\
bcai\_bertl\_pass    & 0.748 & 0.762 & 23 \\
nlm-ens-bst-2        & 0.743 & 0.759 & 28 \\
fr\_pass\_roberta    & 0.733 & 0.758 & 20 \\
bigIR-BERT-R         & 0.728 & 0.758 & 19 \\
bigIR-T5-R           & 0.750 & 0.755 & 24 \\
1                    & 0.728 & 0.755 & 18 \\
p\_bm25rm3\_duo      & 0.739 & 0.754 & 8  \\
nlm-ens-bst-3        & 0.735 & 0.753 & 29 \\
nlm-bert-rr          & 0.722 & 0.750 & 30 \\
bigIR-T5xp-T5-F      & 0.735 & 0.745 & 27 \\
2                    & 0.730 & 0.744 & 25 \\
bigIR-DCT-T5-F       & 0.733 & 0.741 & 21 \\
relemb\_mlm\_0\_2    & 0.724 & 0.739 & 31 \\
nlm-prfun-bert       & 0.730 & 0.728 & 32 \\
TUW-TK-2Layer        & 0.739 & 0.722 & 34 \\
p\_d2q\_bm25         & 0.713 & 0.699 & 35 \\
p\_d2q\_bm25rm3      & 0.693 & 0.693 & 36 \\
bert\_6              & 0.726 & 0.691 & 37 \\
TUW-TK-Sparse        & 0.700 & 0.682 & 33 \\
CoRT-bm25            & 0.694 & 0.664 & 38 \\
indri-fdm            & 0.709 & 0.652 & 43 \\
bl\_bcai\_mdl1\_vt   & 0.707 & 0.650 & 40 \\
terrier-DPH          & 0.689 & 0.650 & 52 \\
indri-lmds           & 0.702 & 0.649 & 47 \\
terrier-InL2         & 0.693 & 0.649 & 44 \\
bcai\_class\_pass    & 0.694 & 0.647 & 41 \\
indri-sdm            & 0.698 & 0.642 & 48 \\
terrier-BM25         & 0.683 & 0.641 & 45 \\
DLH\_d\_5\_t\_25     & 0.650 & 0.641 & 46 \\
% bl\_bcai\_mdl1\_vs   & 0.681 & 0.636 & 42 \\
% CoRT-standalone      & 0.676 & 0.630 & 39 \\
% p\_bm25rm3           & 0.637 & 0.625 & 49 \\
% TF\_IDF\_d\_2\_t\_50 & 0.663 & 0.619 & 53 \\
% p\_bm25              & 0.650 & 0.598 & 50 \\
% bm25\_bert\_token    & 0.667 & 0.585 & 51 \\
% small\_1k            & 0.635 & 0.490 & 54 \\
% med\_1k              & 0.646 & 0.474 & 55 \\
% DoRA\_Large\_1k      & 0.633 & 0.468 & 56 \\
 $\dots$ & $\dots$ & $\dots$& $\dots$ \\
DoRA\_Small          & 0.285 & 0.182 & 57 \\
DoRA\_Large          & 0.278 & 0.171 & 59 \\
DoRA\_Med            & 0.270 & 0.171 & 58 \\
\midrule
  &     &          &       \texttt{Sun} / \texttt{Fag} / \texttt{Thom}                          \\
Spearman Correlation & 0.88  & 0.96      &        0.96 / 0.95 / 0.95                      \\
Kendall Correlation  & 0.70   & 0.84      &        0.88 / 0.85 / 0.84 \\     
\bottomrule
\end{tabular}
\end{small}
\end{table}

==> results/exam_post_pipeline-analysis.txt.tex <==

\section{CAR Y3 - TQA / Answer checking }

\begin{verbatim}

## Inter-annotator

# squad2-finetuned model name:  sjrhuschlee/flan-t5-large-squad2



### Use T5 answer corrected files   ###

QA/Squad2:
result_car_qa="/mnt/cherries/datasets/trec-car-data/additional/answerT5corrected_squad2-t5-qa-tqa-exam--benchmarkY3test-exam-qrels-runs-with-text.jsonl.gz"

# QA
exp="car-tqa-qa-v5"
prompt="QuestionCompleteConcisePromptWithT5VerifiedAnswerKey2"
python -O -m exam_pp.exam_post_pipeline $result_car_qa  --prompt-class $prompt --question-set tqa  --testset cary3   --model google/flan-t5-large --leaderboard-out "leaderboard-${exp}.tsv" --correlation-out "correlation--${exp}.tex" --qrel-query-facets -q "qrel-${exp}.qrels"  > "${exp}-analysis.log"

#min_rating=None nExam:CorrelationStats(spearman_correlation=0.7313103409735259, kendall_correlation=0.5493612827995783)
# min_rating=None  exam:CorrelationStats(spearman_correlation=0.7150261026117674, kendall_correlation=0.5321937427120915)



#Squad2
exp="car-tqa-squad2-v5"
prompt="QuestionCompleteConcisePromptWithT5VerifiedAnswerKey2"
python -O -m exam_pp.exam_post_pipeline $result_car_qa  --prompt-class $prompt --question-set tqa  --testset cary3   --model sjrhuschlee/flan-t5-large-squad2 --leaderboard-out leaderboard-${exp}.tsv --correlation-out correlation--${exp}.tex  --qrel-query-facets -q "qrel-${exp}.qrels" > "${exp}-analysis.log"

min_rating=None nExam:CorrelationStats(spearman_correlation=0.8660254037844386, kendall_correlation=0.7553717638494203)
min_rating=None  exam:CorrelationStats(spearman_correlation=0.8630646331732098, kendall_correlation=0.7382042237619334)


# CC:
result_car_cc="/mnt/cherries/datasets/trec-car-data/additional/answerT5corrected_t5-rating-naghmehs-tqa-rating-cc-exam-qrel-runs-result.jsonl.gz"

exp="car-tqa-cc-v5"
prompt="QuestionCompleteConcisePromptWithT5VerifiedAnswerKey2"
python -O -m exam_pp.exam_post_pipeline $result_car_cc  --prompt-class $prompt --question-set tqa  --testset cary3   --model google/flan-t5-large --leaderboard-out leaderboard-${exp}.tsv --correlation-out correlation--${exp}.tex  --qrel-query-facets -q "qrel-${exp}.qrels" > "${exp}-analysis.log"

min_rating=None nExam:CorrelationStats(spearman_correlation=0.877868486229354, kendall_correlation=0.7210366836744466)
min_rating=None  exam:CorrelationStats(spearman_correlation=0.877868486229354, kendall_correlation=0.7210366836744466)

## ---



Use nltk answer corrected files

QA/Squad2:  answercorrected-squad2-t5-qa-tqa-exam--benchmarkY3test-exam-qrels-runs-with-text.jsonl.gz
CC: answercorrected-t5-rating-naghmehs-tqa-rating-cc-exam-qrel-runs-result.jsonl.gz
--prompt-class QuestionCompleteConcisePromptWithAnswerKey2


--------------

Anwer corrected

QA/Squad2:

result_car_qa="/mnt/cherries/datasets/trec-car-data/additional/answercorrected-squad2-t5-qa-tqa-exam--benchmarkY3test-exam-qrels-runs-with-text.jsonl.gz"
result_car_qa="answercorrected-squad2-t5-qa-tqa-exam--benchmarkY3test-exam-qrels-runs-with-text.jsonl.gz"

# QA
exp="car-tqa-qa-corrected"
prompt="QuestionCompleteConcisePromptWithAnswerKey2"
python -O -m exam_pp.exam_post_pipeline $result_car_qa  --prompt-class $prompt --question-set tqa  --testset cary3   --model google/flan-t5-large --leaderboard-out "leaderboard-${exp}.tsv" --correlation-out "correlation--${exp}.tex" --qrel-query-facets -q "qrel-${exp}.qrels"  > "${exp}-analysis.log"

mkdir datax
ls *${exp}*
cp *${exp}* datax/


#Squad2
exp="car-tqa-squad2-corrected"
prompt="QuestionCompleteConcisePromptWithAnswerKey2"
python -O -m exam_pp.exam_post_pipeline $result_car_qa  --prompt-class $prompt --question-set tqa  --testset cary3   --model sjrhuschlee/flan-t5-large-squad2 --leaderboard-out "leaderboard-${exp}.tsv" --correlation-out "correlation--${exp}.tex" --qrel-query-facets -q "qrel-${exp}.qrels"  > "${exp}-analysis.log"
cp *${exp}* datax/

# CC:
# result_car_cc="/mnt/cherries/datasets/trec-car-data/additional/answercorrected-t5-rating-naghmehs-tqa-rating-cc-exam-qrel-runs-result.jsonl.gz"
result_car_cc="answercorrected-t5-rating-naghmehs-tqa-rating-cc-exam-qrel-runs-result.jsonl.gz"

exp="car-tqa-cc-corrected"
prompt="QuestionCompleteConcisePromptWithAnswerKey2"
python -O -m exam_pp.exam_post_pipeline $result_car_cc  --prompt-class $prompt --question-set tqa  --testset cary3   --model google/flan-t5-large --leaderboard-out leaderboard-${exp}.tsv --correlation-out correlation--${exp}.tex  --qrel-query-facets -q "qrel-${exp}.qrels" > "${exp}-analysis.log"

cp *${exp}* datax/

% -------------

% #### Correlation/Leaderboard #####

% #Squad2

% python -O -m exam_pp.exam_post_pipeline $result_car_qa  --prompt-class QuestionCompleteConcisePromptWithAnswerKey2 --question-set tqa  --testset cary3 --model sjrhuschlee/flan-t5-large-squad2 --leaderboard-out leaderboard-car-tqa-squad2.tsv 


% Exam-Cover leaderboard (answer-corrected)
% CC
% min_rating=None  exam:CorrelationStats(spearman_correlation=0.9370838984539311, kendall_correlation=0.8412094642868543)


% QA 
% min_rating=None  exam:CorrelationStats(spearman_correlation=0.8230942299216203, kendall_correlation=0.6695340634119862)

% Squad2
% min_rating=None  exam:CorrelationStats(spearman_correlation=0.8378980829777646, kendall_correlation=0.6867016034994731)



% ************************
% *  Bug in code, all 0! *
% ************************


\end{verbatim}





\section{CAR Y3 - TQA}
\begin{verbatim}
#result_car="/mnt/cherries/datasets/trec-car-data/additional/t5-rating-naghmehs-tqa-exam-qrel-runs-result.jsonl.gz"
#result_car="/mnt/cherries/datasets/trec-car-data/additional/answercorrected-t5-rating-naghmehs-tqa-exam-qrel-runs-result.jsonl.gz"

runs_car="/mnt/cherries/datasets/trec-car-data/benchmarkY3test-runs-and-more/run/"


#### EXAM-Qrels  #### 
not applicable (because we have faceted run files, but no faceted qrels)


#### Inter-annotator ######
# TQA

# Use Ratings

python -O -m exam_pp.exam_post_pipeline $result_car --correlation-out correlation-car-tqa-self-rating.tex --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set tqa  --testset cary3  --use-ratings 

using min_answers=2: ./result/correlation-car-tqa-self-rating--min-answers-2.tex 


#### Leaderboard Correlation ######
# TQA

# Use Self-ratings
exp="car-tqa-self-rating"
python -O -m exam_pp.exam_post_pipeline $result_car --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set tqa  --testset cary3  --use-ratings   --leaderboard-out leaderboard-${exp}$-4.tsv --min-self-rating 4  --correlation-out correlation-${exp}.tex


min_rating=4 nExam:CorrelationStats(spearman_correlation=0.9252408160090155, kendall_correlation=0.789706844024394)
min_rating=4  exam:CorrelationStats(spearman_correlation=0.9222800453977867, kendall_correlation=0.7725393039369071)

./results/leaderboard-car-tqa-self-rating-4.tsv

Column TQA/Exam in latex table ./result/car-y3-leaderboard-correlation.tex

## CompleteAndConcise

% grading more runs with this command
% stdbuf -oL -eL  python -m exam_pp.exam_grading  -o t5-rating-naghmehs-tqa-rating-cc-exam-qrel-runs-result.jsonl.gz  $result_car --model-pipeline text2text --model-name google/flan-t5-large --prompt-class QuestionCompleteConcisePromptWithAnswerKey --question-path ./tqa_train_val_test --question-type tqa >examscore.log 2>&1  &



\end{verbatim}


\section{CAR Y3 - Davinci }

\begin{verbatim}
result_davinci_car="/mnt/cherries/datasets/trec-car-data/additional/davinci-cc-self-rated-naghmeh--cc-self-rated-tqa--exam.jsonl.gz"


# self-rating

python -O -m exam_pp.exam_post_pipeline $result_davinci_car --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set tqa  --testset cary3  --use-ratings   --leaderboard-out leaderboard-davinci-tqa-self-rating-4.tsv --min-self-rating 4 --official-leaderboard empty_leaderboard.json

python -O -m exam_pp.exam_post_pipeline $result_davinci_car --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set naghmeh  --testset cary3  --use-ratings   --leaderboard-out leaderboard-davinci-naghmeh-self-rating-4.tsv --min-self-rating 4 --official-leaderboard empty_leaderboard.json


# cc

python -O -m exam_pp.exam_post_pipeline $result_davinci_car --use-ratings  --prompt-class QuestionCompleteConcisePromptWithAnswerKey --question-set tqa  --testset cary3    --leaderboard-out leaderboard-davinci-tqa-cc.tsv --official-leaderboard empty_leaderboard.json


************************
*  Bug in code, all 0! *
************************

python -O -m exam_pp.exam_post_pipeline $result_davinci_car --use-ratings  --prompt-class QuestionCompleteConcisePromptWithAnswerKey --question-set naghmeh  --testset cary3    --leaderboard-out leaderboard-davinci-tqa-cc.tsv --official-leaderboard empty_lea


************************
*  Bug in code, all 0! *
************************


\end{verbatim}

\section{CAR Y3 - GenQuestions}

\begin{verbatim}
% result_car="/mnt/cherries/datasets/trec-car-data/additional/t5-rating-naghmehs-exam-qrel-runs-result.json.gz"
result_car="/mnt/cherries/datasets/trec-car-data/additional/answercorrected-t5-rating-naghmehs-tqa-rating-cc-exam-qrel-runs-result.jsonl.gz"

runs_car="/mnt/cherries/datasets/trec-car-data/benchmarkY3test-runs-and-more/run/"

## EXAM-Qrels, Inter-annotator, Leaderboard 

exp="car-naghmeh-self-rating"
 python -O -m exam_pp.exam_post_pipeline $result_car --use-ratings -q qrel-${exp}.qrels --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set naghmeh  --testset cary3 --qrel-query-facets --use-ratings  --run-dir $runs_car  --correlation-out correlation-${exp}.tex --leaderboard-out leaderboard-${exp}-4.tsv --min-self-rating 4 --qrel-leaderboard-out qrel-leaderboard-${exp}.tsv > ${exp}-analysis.log

 
% #### EXAM-Qrels  #### 

% # Naghmeh's question set  (using facets)

%  python -O -m exam_pp.exam_post_pipeline $result_car --use-ratings -q out-complete.qrels --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set naghmeh  --testset cary3 --qrel-query-facets --use-ratings  --run-dir $runs_car
 



% #### Inter-annotator ######
% # Naghmeh's questions

% python -O -m exam_pp.exam_post_pipeline $result_car --correlation-out correlation-car-naghmeh-self-rating.tex --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set naghmeh  --testset cary3  --use-ratings 

% using min_answers=2:  /results/correlation-car-naghmeh-self-rating--min-answers-2.tex



% #### Leaderboard Correlation ######
% # Naghmeh's questions

% # Use Self-ratings

% python -O -m exam_pp.exam_post_pipeline $result_car --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set naghmeh  --testset cary3  --use-ratings   --leaderboard-out leaderboard-car-naghmeh-self-rating-4.tsv --min-self-rating 4


% min_rating=4 nExam:CorrelationStats(spearman_correlation=0.8689861743956674, kendall_correlation=0.6867016034994731)
% min_rating=4  exam:CorrelationStats(spearman_correlation=0.8689861743956674, kendall_correlation=0.6867016034994731)


% ./results/leaderboard-car-naghmeh-self-rating-4.tsv

% Column GenQ/Exam in latex table ./result/car-y3-leaderboard-correlation.tex


\end{verbatim}

\section{CAR Y3 - flan-t5-small}

\begin{verbatim}

#### Leaderboard Correlation ######
# Naghmeh's questions

# Use Self-ratings

result_car_t5small="/mnt/cherries/datasets/trec-car-data/additional/t5small-rating-naghmeh--exam-qrels-runs.jsonl.gz"

python -O -m exam_pp.exam_post_pipeline $result_car_t5small --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set naghmeh  --testset cary3  --use-ratings   --leaderboard-out leaderboard-car-naghmeh-t5small-self-rating-4.tsv --min-self-rating 4

min_rating=4 nExam:CorrelationStats(spearman_correlation=0.31532207009587254, kendall_correlation=0.29184818148727604)
min_rating=4  exam:CorrelationStats(spearman_correlation=0.31532207009587254, kendall_correlation=0.29184818148727604)

\end{verbatim}



\section {DL19}

\begin{verbatim}

result_dl="/home/nf1104/work/dl19_results_examGrading/result_trecDL2019-qrels-runs-with-text__new_subqueries_v2__large_2.jsonl.gz"

% runs_dl="/home/nf1104/work/trec-dl-2019/runs/dl19_runs" --- this path does not exist
runs_dl="/mnt/cherries/home/nf1104/work/trec-dl-2019/runs"
commands

######



% this command is incomplete
% python -O -m exam_pp.exam_post_pipeline $result_dl --use-ratings -q out-complete.qrels --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set question-bank  --testset dl19  --use-ratings  --run-dir $runs_dl

python -O -m exam_pp.exam_post_pipeline $result_dl --use-ratings -q dl19-exam-3.qrels --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set question-bank  --testset dl19  --use-ratings  --run-dir $runs_dl --min-trec-eval-level 3 --qrel-leaderboard-out leaderboard-dl19-qrels-genq-self-rating-3.tsv



#####

python -O -m exam_pp.exam_post_pipeline $result_dl --correlation-out correlation-dl19-subqueries-self-rating.tex --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set question-bank  --testset dl19  --use-ratings 

 using min_answers=2: /results/correlation-dl19-self-rating--min-answers-2

#######
#######
#######
files with prompts:


exp="dl19"
result_dl19="/home/nf1104/work/prompt_results/prompt_grades_dl19_correct_answered.jsonl.gz"
runs_dl19="/home/nf1104/work/trec-dl-2019/runs"


cls_values=("FagB" "FagB_few" "Sun" "Sun_few" "HELM" "Thomas")
for cls in "${cls_values[@]}"; do
    # Run the command for each cls value
    python -O -m exam_pp.exam_post_pipeline "$result_dl19" \
        --use-relevance-prompt \
        --trec-eval-qrel-correlation "/home/nf1104/work/qrels/${cls}-${exp}.qrel" \
        --question-set question-bank \
        --testset "$exp" \
        --run-dir "$runs_dl19" \
        --prompt-class "$cls" \
        --correlation-out "./prompted_results/correlation-${cls}-${exp}.tex" \
        --leaderboard-out "./prompted_results/leaderboard-${cls}-${exp}.tsv" \
        --qrel-leaderboard-out "./prompted_results/qrel-leaderboard-${cls}-${exp}.tsv" \
        > "${cls}-analysis.log"
done



#######
exp="dl20"
result_dl20="/home/nf1104/work/prompt_results/prompt_grades_dl20_correct_answered.jsonl.gz"
runs_dl20="/home/nf1104/work/trec-dl-2020/runs"

python -O -m exam_pp.exam_post_pipeline $result_dl20 --use-ratings -q dl20-exam-4.qrels --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set question-bank  --testset dl20  --use-ratings  --run-dir $runs_dl20 --min-trec-eval-level 4 --qrel-leaderboard-out leaderboard-dl20-qrels-genq-self-rating-4.tsv



cls_values=("FagB" "FagB_few" "Sun" "Sun_few" "HELM" "Thomas")

cls_values=("FagB" "FagB_few" "Sun" "Sun_few" "HELM" "Thomas")
for cls in "${cls_values[@]}"; do
    # Run the command for each cls value
    python -O -m exam_pp.exam_post_pipeline "$result_dl20" \
        --use-relevance-prompt \
        --trec-eval-qrel-correlation "/home/nf1104/work/qrels/${cls}-${exp}.qrel" \
        --question-set question-bank \
        --testset "$exp" \
        --run-dir "$runs_dl20" \
        --prompt-class "$cls" \
        --correlation-out "./prompted_results/correlation-${cls}-${exp}.tex" \
        --leaderboard-out "./prompted_results/leaderboard-${cls}-${exp}.tsv" \
        --qrel-leaderboard-out "./prompted_results/qrel-leaderboard-${cls}-${exp}.tsv" \
        > "${cls}-analysis.log"
done
\end{verbatim}

==> worked-example.tex <==
\begin{quote}

\textbf{Query title}: The Integumentary System \\ \textbf{Query subtopic}: Structure of the Skin\\
\textbf{Passage}:\\
\textbf{ID:} \texttt{b95bf325b7fdacac183b1daf7c118be407f52a3a}

The skin is the largest organ in the human body. Skin is made up of three layers, the epidermis, dermis and the fat layer, also called the hypodermis.  \hl{The epidermis is the outer layer of skin that keeps} vital fluids in and \hl{harmful bacteria out of the body}.  \hl{The dermis is the inner layer of skin} that contains \hl{blood vessels}, \hl{nerves}, hair follicles, oil, and \hl{sweat glands}. Severe damage to large areas of skin exposes the human organism to dehydration and infections that can result in death.\\
\textbf{TREC judgment}: 3 (MUST be mentioned)\\
\end{quote}

% \begin{itemize}
%     \item \textbf{\genQ{}:}
%     \begin{itemize}
%         \item[q1?] How does the epidermis, dermis, and hypodermis work together to provide protection, sensation, and regulation for the body?\newline
%         [EXAM Score] "4"
        
%         % \item[q2?] Can the integumentary system be compromised by diseases and conditions, and if so, how does this impact the health of the skin?\newline
%         % [EXAM Score] "4"
        
%         % \item[q3?] How does the skin act as a barrier against pathogens and other foreign substances?\newline
%         % [EXAM Score] "4"
%     \end{itemize}
    
%     \item \textbf{TQA Questions:}
%     \begin{itemize}
    
%         \item[]NDQ\_007535 Outer layer of the skin \newline
%         [EXAM Score] "4" \newline
%         [Answer] epidermis
%     \end{itemize}
% \end{itemize}

